Prototypical Recurrent Unit

Despite the great successes of deep learning, the effectiveness of deep neural networks has not been understood at any theoretical depth. This work is motivated by the thrust of developing a deeper understanding of recurrent neural networks, particularly LSTM/GRU-like networks. As the highly complex structure of the recurrent unit in LSTM and GRU networks makes them difficult to analyze, our methodology in this research theme is to construct an alternative recurrent unit that is as simple as possible and yet also captures the key components of LSTM/GRU recurrent units. Such a unit can then be used for the study of recurrent networks and its structural simplicity may allow easier analysis. Towards that goal, we take a system-theoretic perspective to design a new recurrent unit, which we call the prototypical recurrent unit (PRU). Not only having minimal complexity, PRU is demonstrated experimentally to have comparable performance to GRU and LSTM unit. This establishes PRU networks as a prototype for future study of LSTM/GRU-like recurrent networks. This paper also studies the memorization abilities of LSTM, GRU and PRU networks, motivated by the folk belief that such networks possess long-term memory. For this purpose, we design a simple and controllable task, called ``memorization problem'', where the networks are trained to memorize certain targeted information. We show that the memorization performance of all three networks depends on the amount of targeted information, the amount of ``interfering" information, and the state space dimension of the recurrent unit. Experiments are also performed for another controllable task, the adding problem, and similar conclusions are obtained.

==> catchall.tex <==
\section{TO DO LIST}

\subsection{Dingkun}



\begin{itemize}

\item What is the choice of activation function $h$ in each experiment for PRU. 

\item Plots may contain missing information.

\item Now: what are the noise variances in Figure \ref{fig:overall_MP} and in Figure \ref{fig:problem_MP}?

\item Now: make three plots, comparing the time complexity of the three units (similar to the three plots in Figure \ref{fig:overall_MP}).

\item (done) Now: Check, for memorization problem, does there exist a case where PRU with state dimension $K$ performs the same as or better than GRU with state dimension $K'$, where $K>K'$. 

\item Future research: Prove that for PRU, no need to have output dimension higher than state dimension. 

\item Full paper: include a structural comparison with LSTM and GRU

\end{itemize}
